Survival of the strictest: Stable and unstable equilibria under regularized learning with partial information

In this paper, we examine the Nash equilibrium convergence properties of no-regret learning in general N-player games. For concreteness, we focus on the archetypal follow the regularized leader (FTRL) family of algorithms, and we consider the full spectrum of uncertainty that the players may encounter - from noisy, oracle-based feedback, to bandit, payoff-based information. In this general context, we establish a comprehensive equivalence between the stability of a Nash equilibrium and its support: a Nash equilibrium is stable and attracting with arbitrarily high probability if and only if it is strict (i.e., each equilibrium strategy has a unique best response). This equivalence extends existing continuous-time versions of the folk theorem of evolutionary game theory to a bona fide algorithmic learning setting, and it provides a clear refinement criterion for the prediction of the day-to-day behavior of no-regret learning in games

==> results-MV.tex <==
%
%
%
%


To understand the long-run behavior of \eqref{eq:FTRL}, we will focus on the following overarching question:
\emph{Which \aclp{NE} hold convergence and stability properties and how are these properties affected by the uncertainty in the players' feedback model?}
%

We begin by providing the technical groundwork for our results in \cref{sec:stability} below;
subsequently, we state and discuss our main results in \cref{sec:results}, postponing the technical analysis and proofs to \cref{sec:}.


\subsection{Asymptotic Stability}
\label{sec:stability} 

%
\AG{Changed the paragraph}
To address this question the precise definition of stability is sine qua non. %
First observe that  global stability results are not of interest,
since FTRL's time evolution depends on its initialization and a game may admit several Nash equilibria. %
 Thus, we focus on the notion of \emph{asymptotic stability}, the standard criterion in the literature for the characterization of local stability. %
 Roughly speaking, a point is asymptotically stable if, whenever the sequence of play starts "close enough", remains "close enough" and finally converges to it \AG{Not sure about this sentence}. However, in stochastic algorithms stability guarantees become more intricate; if the players’ payoff information is incomplete, a single unlucky estimation could drive $\pstate_\run$ away from the basin of a \acl{NE}, possibly never to return. As a result, any local convergence result under uncertainty must be probabilistic in nature. %
For getting around this negative result "almost surely"  is turned into "with arbitrarily high probability" leading to the definition of stochastic asymptotic stability.
%
\begin{definition}[Stochastic Asymptotic Stability]\label{stability} Fix a confidence level $\conlevel >0$. We say that $\eq\in\pspace$ is:
\begin{enumerate}[topsep=.5ex,leftmargin=\parindent]
\setlength{\itemsep}{0pt}
\setlength{\parskip}{.2ex}
    \item \emph{Stable}: For each neighborhood $V$ of $\eq$, there exists neighborhood $U$ of $\eq$, such that  with probability at least $1-\conlevel$, $\pstate_\run \in V$ for all $\run \geq 0$, whenever $\pstate_0 \in U\cap \im\mirror$. Equivalently, if $\pstate_0\in U \cap\im\mirror$ then 
\begin{equation}
    \probof{\pstate_\run\in V\;\; \forall \run\geq 0 }\geq 1-\conlevel
\end{equation}
\item \emph{Attracting}:  There exists neighborhood $U$ of $\eq$ such that whenever $\pstate_0 \in U\cap\im\mirror$ then 
\begin{equation}
    \probof{\lim_{\run\to\infty}\curr =\eq}\geq 1-\conlevel
\end{equation}
\item \emph{Stochastically Asymptotically Stable}: if it is stable and attracting.
\end{enumerate}
\end{definition}
\begin{remark}\label{stability remark}
In the definition above, we demand $\pstate_0 \in U\cap \im\mirror$ to pinpoint that some points of the boundary may be infeasible as initial states. Looking at the two examples, \cref{MWU,Projection} there is a dichotomy in the properties of the corresponding mirror maps. On the one hand, the kernel of the Euclidean/quadratic regularizer is differentiable in all of $[0,1]$. On the other hand, the derivative of the kernel of the negative Shannon-entropy goes to $\infty$ as $x$ goes to $0$. %
This means that in the latter the boundaries are off the limits and inevitably some initial conditions do not belong in $\im\mirror$. This dichotomy is extensively discussed in \cref{ss:steep vs non-steep}.
\end{remark}
\noindent We are now ready to state our main results:




\subsection{Main Results}%
\label{sec:statements}

\begin{theorem}\label{theorem:if}
Let $\eq$ be a strict \acl{NE}. If \eqref{eq:FTRL} is run with payoff feedback that satisfies assumptions \ref{asm:bias}-\ref{asm:variance} %
then $\eq$ is stochastically asymptotically stable.
\end{theorem}
\begin{theorem}\label{theorem:only-if}

Let $\eq$ be a mixed \acl{NE}. If \eqref{eq:FTRL} is run with payoff feedback that satisfies assumption \ref{asm:degen} then $\eq$ is not stochastically asymptotically stable for any choice of the parameters of the algorithm.
\end{theorem}
\begin{center}
\begin{tcolorbox}[enhanced,width=0.95\textwidth, drop fuzzy shadow southwest, 
                    boxrule=0.4pt,colframe=black!80!black,colback=black!10]\label{main theorem}
\vspace{0.1cm}
{\textbf{Main Theorem.}\emph{
Let $\eq$ be a Nash equilibrium. Then %
 %
 under assumptions \ref{asm:bias}-\ref{asm:degen} $\eq$ is stochastically asymptotically stable $\Leftrightarrow$ $\eq$ is a strict Nash equilibrium.}}
\end{tcolorbox}
\end{center}
%
\begin{corollary}\AG{Think here we have to put $\sum_n\step_n^2 <\infty$, since it is needed to osatisfy the assumptions.}
If \eqref{eq:FTRL} is run with feedback described in \cref{semibandit feedback} %
and the game is generic, then a \acl{NE} is stochastically asymprotically stable, if and only if it is a strict \acl{NE}.
\end{corollary}

\begin{corollary}
If \eqref{eq:FTRL} is run with feedback described in \cref{bandit feedback} with %
$\sum_\run \step_\run^2/\epar_\run <\infty$, $\sum_\run \step_\run \epar_\run <\infty$ and the game is generic, then a \acl{NE} is stochastically asymptotically stable, if and only if it is a strict \acl{NE}.
\end{corollary}
\noindent To the best of our knowledge our result is the first one to provide stability guarantees for the bandit framework in general $N-$players games.
\section{Our Techniques}\label{sec:Proof Techniques}
We begin by giving a high level overview of  \Cref{theorem:if}, namely the necessary conditions that \eqref{eq:FTRL} should satisfy such that strict Nash equilibria are stochastically asymptotically stable.  Having established our first stability result, then we explore the main ideas behind instability of mixed Nash equilibria  \Cref{theorem:only-if} and its associated proof of correctness.
%
%
\subsection{The Stochastic Asymptotic Stability of Strict Nash Equilibria}\label{sec:Stability:Proof Techniques}
At the highest level, the standard tool in FTRL dynamics for questions pertaining to asymptotic stability of strict \aclp{NE} is the construction of a potential function, well-known as \emph{Second Lyapunov's method}. However, the analysis and the underlying structural results are considerably more involved when we shift from the continuous dynamics to discrete algorithms and more importantly in a stochastic framework with incomplete feedback information. Still, to built intuition we first recall the continuous and deterministic analogue. 
\subparagraph{The continuous time.}
%
In prior work \citep{HS75,Wei00,Har11}, multiple instantiations of Bregman functions, like the KL-divergence  have been employed as a potent tool for understanding  \emph{replicator \& population dynamics}, which are the continuous analogues of MWU/EW (\cref{MWU}). 
Unfortunately, Bregman functions are  insufficient  to cover the full spectrum of regularizers studied in this work. %
 %
 This limitation has been sidesteped in \cite{MS16} by exploiting the information of the dual space $\dspace$ of the payoff scores,  via the Fenchel coupling: %
\begin{equation}
\fench_\hreg\parens{x,y}  = \hreg\parens{x} + \hreg^*\parens{y} -\inner{y}{x} \text{ for all } x\in\pspace, y\in\dspace
\end{equation}   
where $\hreg^*: \dspace \to \R$ is the convex conjugate
%
of $\hreg$: $\hreg^*\parens{y} = \sup_{x\in\pspace}\braces{\inner{y}{x} -\hreg\parens{x}}$. 
Indeed,\AG{Changed it see how it looks} %
$\fench_\hreg\parens{\eq,y}\ge 0$ where equality holds if and only if $\eq=Q(y)$ (\cref{prop:Prop Fenchel}).
Therefore,  for the continuous FTRL dynamics $\dot{y}(t)=v(x(t)), x(t)=Q(y(t))$, it remains to show that  the time derivative of the Lyapunov-candidate-function $L_{\eq}(y(t))=\fench_\hreg\parens{\eq,y(t)}$ is negative. %
This last key ingredient for the strict Nash equilibria is derived by their \emph{variational stability} property. 

\noindent Formally, a point $\eq$ is \emph{variationally stable} if there exists a neighborhood $U$ of $\eq$ such that 
\begin{equation}\label{variational stability-main}
     \inner{\payv\parens{x}}{x-\eq}\leq 0 \text{ for all  }x\in U \tag{VS}
\end{equation}
with equality if and only if $x=\eq$. Roughly speaking, this property states that the payoff vectors are pointing ``towards'' the equilibrium in question since in a neighborhood of $\eq$, it strictly dominates over all other strategies. Thus by applying the chain rule, \eqref{variational stability-main} implies that ${\mathrm{d} L_{\eq}(y(t))}/{\mathrm{d} t}\leq 0$
\footnote{Analytically, $\dfrac{\mathrm{d} L_{\eq}(y(t))}{\mathrm{d} t}=\dfrac{\mathrm{d}{\hreg^*\parens{y(t)}}}{\mathrm{d} t} -\inner{\dot{y}(t)}{\eq}= \inner{\dot{y}(t)}{\nabla\hreg^*\parens{y}} -\inner{\dot{y}(t)}{\eq}= \inner{\payv\parens{x(t)}}{x(t)-\eq}\leq 0.
$%
}.
\noindent Given their usefulness also in the discrete time stochastic case, we present all the aformentioned properties in detail 
%
in the paper’s supplement (\cref{ss:Bregman}-\ref{ss:variational stability}).

\subparagraph{The discrete time.}
The core elements of the continuous time proof do not trivially extend to the discrete time case.
%
Even though  we are not able to show that $\parens{\fench_\hreg\parens{\eq,\dstate_\subround}}_{\subround=1}^{\infty}$ is a decreasing sequence, due to the discretization and the uncertainty involved, we prove that $ \fench_\hreg\parens{\eq,\dstate_\subround} \to 0$. This immediately implies that FTRL algorithm converges to $\eq$, since from \cref{prop:Prop Fenchel} $\fench_\hreg\parens{\eq,\dstate_\subround}\ge \frac{1}{2\stcon_\hreg}\norm{\eq-\pstate_\subround}$.


%
%

To exploit again the Fenchel coupling as a Lyapunov function, successive differences have to be taken among 
$\fench_\hreg\parens{\eq,\dstate_{\round+1}}, \ldots, \fench_\hreg\parens{\eq,\dstate_{0}}$.
%
In contrast to the continuous time analysis, since the chain rule no longer applies, we can only do a second order Taylor expansion of the Fenchel coupling. 
Additionally, let us recall that in our stochastic feedback model, the payoff vector $\npayv_\round= \payv\parens{\pstate_\round}+\noise_\round + \bias_\round$ including possibly either random zero-mean noise or systematic biased noise.
Combining \cref{prop:Prop Fenchel}, definition of $\npayv_\round$ and \eqref{eq:FTRL}, we can create the following upper-bound of Fenchel coupling at each round:
%
%
%
%
%
%
%
%
%
%
%
\begin{equation}\label{fenchel-telescopic-main}
     \fench_\hreg\parens{\eq,\dstate_{\round+1}} \leq \fench_\hreg\parens{\eq,\dstate_0} + \sum_{\subround =0}^\round \step_\subround(\rvdrift_\subround+\rvnoise_\subround+\rvbias_\subround)  + \dfrac{1}{2\stcon_\hreg}\sum_{\subround =0 }^\round \step_\subround^2\norm{\npayv_\subround}_*^2
\tag{$\star$}
\end{equation}
\smallskip
where $\rvdrift_\subround=\inner{\payv\parens{\pstate_\subround}}{\pstate_\subround - \eq},
\rvnoise_\subround=\inner{{\noise_\subround}}{\pstate_\subround - \eq},
\rvbias_\subround=\inner{{\bias_\subround}}{\pstate_\subround - \eq}
$ are the related terms with the drift of the actual payoff, the zero-mean noise and the bias correspondingly.
%
When $\pstate_\round$ lies in a variationally stable region $U_{\ref{variational stability-main}}$ of $\eq$,
%
the first-order term of $\rvdrift_\subround$, which also appears in the continuous time, corresponds actually to the negative ``drift'' of the variational stability which attracts Fenchel coupling to zero. 
%
%
%
%
%
%
%
%
%
%

Having settled the basic framework, we split the proof sketch of \Cref{theorem:if} into two parts: \emph{stochastic stability} \& \emph{convergence}. Our analysis relies heavily on tools from the convex analysis and martingale limit theory to control the influence of the stochastic terms in the aforementioned bound.
\smallskip

\noindent\textbf{Step 1: \emph{Stability}.} Let $U_\eps = \braces{x: \breg_\hreg\parens{\eq,x}<\eps}$ and $U_\eps^* = \left\{y\in\dspace: \fench_\hreg\parens{\eq,y} < \eps\right\}$ be the $\eps-$sublevel sets of Bregman function and  Fenchel coupling respectively. Our first observation is that for all ``natural'' decomposable regularizers, it holds  the so-called ``reciprocity condition'' (\cref{prop:rec Bregman,prop:rec Fencel}): essentially, this posits that $U_\eps$ and $Q(U_\eps^*)$ are neighborhoods of $\eq$ in $\strats$. 
Additionally, since $\fench_\hreg\parens{\eq,y} = \breg_\hreg\parens{\eq,x}$ whenever $\mirror\parens{y}=x$ and $\supp\parens{x}$ contains $\supp\parens{\eq}$, from \cref{prop:Prop Fenchel}, it holds that  $\mirror\parens{U_\eps^*}\subseteq U_\eps$ and $\mirror^{-1}\parens{U_\eps}= U_\eps^*$. Thus, we conclude that whenever $y\in U_\eps^*$, $x=\mirror\parens{y}\in U_\eps$.
\begin{comment}
To proceed, fix a confidence level $\conlevel$ and $\eps$ sufficiently small such that \eqref{variational stability-main} holds for all $x \in U_{\eps}$.
Using Doob's maximal inequalities  %
for (sub)martingales (\cref{Max inequality martingales,Max inequality submartingales}) we can prove that 
\begin{enumerate*}[(a)]\item ${\displaystyle\sup_{\round\in \mathbb{N}}}\{\sum_{\subround =0}^\round \step_\subround\rvnoise_\subround\}$, \item ${\displaystyle\sup_{\round\in \mathbb{N}}}\{\sum_{\subround =0}^\round \step_\subround\rvbias_\subround\}$ and \item ${\displaystyle\sup_{\round\in \mathbb{N}}} \{\frac{1}{2\stcon_\hreg}\sum_{\subround =0 }^\round \step_\subround^2\norm{\npayv_\subround}_*^2\}$\end{enumerate*} are greater or equal $\eps/4$ with probability less than $\delta/3$. 
\smallskip

\noindent Thus, with probability $1-\delta$ it holds that 
\begin{enumerate*}[(a)]\item %
$\sum_{\subround =0}^\round \step_\subround\rvnoise_\subround<\eps/4$, \item %
$\sum_{\subround =0}^\round \step_\subround\rvbias_\subround<\eps/4$ and \item %
%
$\frac{1}{2\stcon_\hreg}\sum_{\subround =0 }^\round \step_\subround^2\norm{\npayv_\subround}_*^2<\eps/4$\end{enumerate*},for all $\round\ge 0$.
Then, martingale bounds are applied by demanding step-size such that $ \sum_{\subround=0}^\infty\step_\subround^2\sbound_\subround^2\leq \bigoh\parens{\eps^2\conlevel}$ and $\sum_{\subround=0}^\infty\step_\subround\bbound_\subround \leq \bigoh\parens{\eps\conlevel}
$.
%
For concision, we defer the full proof to the supplement of the paper in \cref{sec:deferred proofs-of main lemmas}.
\smallskip
\end{comment}

To proceed, fix a confidence level $\conlevel$ and $\eps$ sufficiently small such that \eqref{variational stability-main} holds for all $x \in U_{\eps}$.
Using Doob's maximal inequalities  %
for (sub)martingales (\cref{Max inequality martingales,Max inequality submartingales}) we can prove that  with probability at least $1-\delta$,
\begin{enumerate*}[(a)]\item\label{item:noise} $\{\sum_{\subround =0}^\round \step_\subround\rvnoise_\subround\}$, \item \label{item:bias}$
\{\sum_{\subround =0}^\round \step_\subround\rvbias_\subround\}$ and \item \label{item:discrete-error}$ \{\frac{1}{2\stcon_\hreg}\sum_{\subround =0 }^\round \step_\subround^2\norm{\npayv_\subround}_*^2\}$\end{enumerate*} are less than $\eps/4$ for all $\round\ge 0$. 
For concision, we defer the full proof to the supplement of the paper in \cref{sec:deferred proofs-of main lemmas}. For the rest of this part, we condition on this event and rewrite \eqref{fenchel-telescopic-main} as $\fench_\hreg\parens{\eq,\dstate_{\round+1}} < \sum_{\subround =0}^\round \step_\subround\rvdrift_\subround+\eps$.
\medskip

\noindent Following the definition of stability (\cref{stability}),  we prove inductively that if  $\pstate_0$ belongs a smaller neighborhood, namely if  $\pstate_0 \in U_{\eps/4}\cap \im\mirror$, then $\pstate_\round$ never escapes $U_\eps$, $\pstate_\round\in U_\eps$ for all $\round\geq 0$.

%
%
%
\begin{itemize}[topsep=.5ex,leftmargin=\parindent]
\setlength{\itemsep}{0pt}
\setlength{\parskip}{.2ex}
    \item  Induction Basis/Hypothesis: Since $\pstate_0 \in U_{\eps/4}\cap \im\mirror$, apparently $\fench_\hreg\parens{\eq,\dstate_0} <\eps/4$ and $\pstate_0 \in U_{\eps}$. Assume that $\pstate_\subround \in U_{\eps}$ for all $0\leq \subround\leq \round$. 
    \item  Induction Step: We will prove that $\dstate_{\round +1}\in U_{\eps}^*$ and consequently $\pstate_{\round+1}\in U_{\eps}$. 
    Since $U_{\eps}$ is a neighborhood of $\eq$ in which \eqref{eq:variational stability} holds  we have that
   $\rvdrift_\subround\leq 0$ for all  $0\leq\subround\leq\round $. Consequently $\fench_\hreg\parens{\eq,\dstate_{\round+1}} < \eps$
    which implies that $\dstate_{\round+1} \in U_{\eps}^*$  or equivalently $\pstate_{\round+1} \in U_{\eps}$.  
\end{itemize}
\smallskip

\noindent\textbf{Step 2: \emph{Convergence}.} A tandem combination of stochastic Lyapunov and variational stability is the following lemma:
\begin{lemma}[Informal statement of \cref{lem:strict remain to neighborhood}]
Let $\eq\in \pures$ be a strict Nash equilibrium. If $\curr[\pstate]$ does not exit a neighborhood $R$ of $\eq$, in which variational stability holds, then  there exists a subsequence $\pstate_{\round_\subround}$ of $\state_\round$ that converges to $\eq$ almost surely.
\end{lemma}
%
\noindent Indeed, if $\state_\round$ is entrapped in a variationally stable region $U_\eps$ of $\eq$ without converging to $\eq$, we can show that $\sum_{\subround=0}^\infty \step_\subround \rvdrift_k \to -\infty$, while comparatively by the law of the large numbers for martingales (\cref{law of large numbers}), the contribution of \ref{item:noise},\ref{item:bias},\ref{item:discrete-error}  is negligible. Thus, in limit \eqref{fenchel-telescopic-main} implies that $0\leq \liminf \fench_\hreg\parens{\eq,\dstate_{\round}}\le  -\infty $, which is a contradiction.

%
Our final ingredient to complete the proof is that $\parens{\fench_\hreg\parens{\eq,\dstate_\subround}}_{\subround=1}^{\infty}$ behaves like an almost supermartingale when it is entrapped in a variationally stable region $U_\eps$ of $\eq$. 
So, by convergence theorem for (sub)-martingales (\cref{Doob's convergence}),  $\parens{\fench_\hreg\parens{\eq,\dstate_\subround}}_{\subround=1}^{\infty}$ actually converges to a random  finite variable. Inevitably though, $\liminf_{\round\to\infty}\fench_\hreg\parens{\eq,\dstate_\round} = \lim_{\round\to\infty} \fench_\hreg\parens{\eq,\dstate_\round} = 0$ and by \cref{prop:Prop Fenchel}, $\mirror\parens{\dstate_\round} = \curr \to \eq$.  


\subsection{The Stochastic Instability of Mixed Nash Equilibria}\label{sec:Instability:Proof Techniques}
%
For the proof of \cref{theorem:only-if}, it is worth mentioning that in this case stability fails for any choice of step-size. We start by focusing on the assumption of non-degeneracy \ref{asm:degen} of theorem's statement.%
%
%
%
%
%
\begin{itemize}[topsep=.5ex,leftmargin=\parindent]
\setlength{\itemsep}{0pt}
\setlength{\parskip}{.2ex}
\item From a game-theoretic perspective, \ref{asm:degen} actually demands that with non-zero probability, %
when players receive the payoffs corresponding to pure strategy profiles, there exists at least one player for whom at least two strategies of the equilibrium have distinct payoff signal. %
Note that if for each player, the payoffs corresponding to two different strategies of $\supp (\eq)$ were all equal \footnote{ when all other players' also employ strategies of the equilibrium} immediately implies a non-generic game with pure \aclp{NE}.
\item To illustrate this assumption in our generic feedback model, suppose that this error term $\error_{\run}$ is  standard normal random noise $\xi_{\run}$.
Indeed, the requirement of \ref{asm:degen} is satisfied since $\probof{\abs{ \payv_{\play, a}\parens{\pstate_{\run}} +\xi_{\play a,\run}-\payv_{\play,b}\parens{\pstate_{\run}}-\xi_{\play b,\run}}\geq 1/|\players| }> 1-\bigoh\left(\exp(-1/|\players|^2)\right)$. Such kind of property can be derived actually for any per-coordinate independent noise since actually the event of two independent coordinates to be exactly equal has zero measure.
\end{itemize}
For the bandit models \cref{semibandit feedback}, \cref{bandit feedback} of the previous section, we show that \ref{asm:degen} is satisfied in \cref{cor:non zero payoff,cor:payoffs bounded} of \cref{appendix instability}. 

Moving on to the proof of \Cref{theorem:only-if}, we start our analysis by connecting the difference of the payoff signal between two pure strategies, with the difference of the changes in the output of the regularizers' kernels, $\theta_\play$:
\begin{lemma}[Informal Statement of \Cref{lem:Useful Expression}]\label{Main:Useful Expression}
Let $\pstate_{\play,\round}$ be the sequence of play in \eqref{eq:FTRL} \ie $\pstate_{\play,\round} =\mirror\parens{\dstate_{\play,\round}}\in\pspace_\play$ of player $\play\in\players$; and for some round $\round \geq 0$ let $a,b\in\supp\parens{\pstate_{\play,\round}}$ be two pure strategies of player $\play\in\players$. Then 
%
 it holds:
\begin{equation*}
   \parensnew{{\theta}'_\play\parens{\pstate_{\play a,\round+1 }} - {\theta}'_\play\parens{\pstate_{\play a,\round }}} - \parensnew{{\theta}'_\play\parens{\pstate_{\play b,\round+1}} - {\theta}'_\play\parens{\pstate_{\play b,\round}}}  = \step_\round\parens{\npayv_{\play a,\round}-\npayv_{\play b,\round}}
\end{equation*}
\end{lemma}

\noindent Assume ad absurdum that a mixed \acl{NE} $\eq$ is stochastically asymptotically stable.
First, since $\eq$ is a mixed strategy profile, there exist at least two pure actions $a,b\in\supp(\eq)$.
Second, the stochastic stability implies that for all $\eps,\conlevel >0$ if $\pstate_0$ belongs to an initial neighborhood $U_{\eps}$, then $\norm{\curr -\eq} <\eps$ for all $\round \geq 0$, with probability at least $1-\conlevel$.
Third, by the triangle inequality for two consecutive instances of the sequence of play $\pstate_{\play,\round},\pstate_{\play,\round+1}$ for any player $\play\in\players$ it holds:
\begin{equation}\label{eq:closeness-per-round}
    |\pstate_{\play a,\round+1 } -\pstate_{\play a,\round }|+|\pstate_{\play b,\round+1 } -\pstate_{\play b,\round }|< \bigoh(\eps) \text{ with probability } 1-\conlevel
\end{equation}
%
Consider $\eps$ sufficiently small, such that the probabilities of the strategies that belong to the support of the equilibrium are bounded away from $0$, for all the points of the neighborhood. Since $\theta_\play$ is continuously differentiable in $(0,1]$, the differences described in \cref{Main:Useful Expression} are bounded from $\bigoh\parens{\eps}$ due to \cref{eq:closeness-per-round}. Thus, if the sequence of play $\curr$ is contained to an  $\eps-$neighborhood of $\eq$, then the difference of the feedback, for any player $\play\in\players$, to two strategies of the equilibrium is $\bigoh\parens{\eps/\step_\round}$ with probability at least $1-\conlevel$:
%
\[
 \probof{
\abs{\npayv_{\play a,\round} - \npayv_{\play b,\round}}= \bigoh\parens{\eps/\step_\round}\given\filter_\round} \geq 1-\conlevel
\]
However, from assumption \ref{asm:degen} for a fixed round $\round$ and some player $\play\in\players$, there exist $\noiselb,\problb>0$ such that:
\[
    \probof{\abs{\npayv_{\play a,\round} - \npayv_{\play b,\round}}\geq \noiselb\given\filter_\round} = \problb>0
\]
Thus by choosing $\eps=\bigoh(\noiselb \step_\round )$ and $\delta=\problb/2$, we obtain a contradiction and our proof is complete.

\section{Discussion}
Our result addresses the stability properties of \aclp{NE} under discrete no-regret algorithms, while taking into account the stochastic nature of real world applications. Predictive power is ensured for the case of bandit learning, where the information is extremely limited; but the  
\AG{Alternative}
Our result addresses the asymptotic behavior of discrete non-deterministic no-regret learning concerning all \aclp{NE}.

%





